In-Situ Behavioral Evaluation for LLM Fairness, Not Standardized-Test Scores

LLM fairness should be evaluated through in-situ behavioral pattern rather than standardized-test Q&A benchmarks. We show that the standardized-test paradigm can be structurally unreliable: surface-level prompt construction choices, although entirely orthogonal to the fairness question being tested, account for the majority of score variance, shift fairness conclusions in both the direction and the magnitude, and result in severe discordance in model rankings. We develop MAC-Fairness, a framework that embeds controlled variation factors into in-situ behavioral evaluation, examining how models' disparate-treatment behaviors shift when identity is varied as part of natural multi-agent conversation. Repurposing standardized-test questions as conversation seeds rather than as the evaluation instrument, we evaluate within-model differences in position persistence (how they hold positions, from the self-perspective) and peer receptiveness (how receptive they are to peers, from the other-perspective) across 8 million conversation transcripts spanning multiple models and identity presence configurations. In-situ behavioral evaluation reveals stable, model-specific, disparate-treatment behavioral signatures that could generalize across different fairness benchmarks, a form of evidence the standardized-test paradigm does not offer.

==> file/main/__latexindent_temp_related_works.tex <==
\section{Related Works}\label{mac-fairness:main:related_works}

\paragraph{LLM Fairness Evaluation}
\looseness=-1
Fairness evaluation in LLMs has evolved from embedding-level measures and controlled template-based tests to broader assessments across tasks and social groups \citep{zhao2018gender,nangia2020crows,parrish2021bbq,smith2022m,tamkin2023evaluating,gallegos2024bias,gupta2024calm,rottger2025safetyprompts}.
Recent work extends fairness evaluation to multi-turn dialogue \citep{fan2025fairmt}, yet the dominant paradigm remains standardized-test Q\&A in which model's answer to the question is evaluation instrument.
Rather than measuring what models say in response to fairness-probing questions, we aim to measure how models behave in multi-agent conversational dynamics.

% \vspace{-1ex}
\paragraph{Multi-Agent Interaction in LLMs}
Multi-agent LLM frameworks have been developed primarily to improve task performance through structured collaboration.
For instance, differentiated roles can coordinate software development \citep{hong2023metagpt}, debate-based protocols aggregate diverse model outputs to boost reasoning accuracy \citep{du2024improving,chen2024reconcile,estornell2024multi,wang2025mixture}.
Another line of work uses multi-agent setups for evaluation itself, most notably the LLM-as-judge paradigm \citep{zheng2023judging}, where interaction serves as a quality filter rather than a production mechanism of behaviors themselves.
Previous research also examines emergent collective phenomena \citep{park2023generative,park2024generative,li2025llm,li2025simulating,tennant2025moral}, positioning agents as proxies for human populations.
\citet{binkyte2025interactional} scores intersectional fairness of agent communication and \citet{li2025single} find persona-induced asymmetries in advocacy and acceptance.

% \vspace{-1ex}
\paragraph{Persona, Role-Playing, and Personalization}
The persona literature in LLMs encompasses both role-playing with assigned identities and personalization to user profiles, with recent advances in scaling persona simulation through curated datasets, evaluation protocols, and optimized role-playing prompts \citep{tseng2024two,wang2025coser,duan2025orpp}.
Persona assignments systematically shift conversational behavior such as empathy and supportiveness, and LLMs can reconstruct broad psychological trait networks from sparse personality inputs, revealing internally structured personality representations \citep{wu2025personas,liu2026five}.
Persona prompts themselves serve as bias probes \citep{cheng2023marked}, with the prompt's format shaping the portrayal \citep{lutz2025prompt}.

% \vspace{-1ex}
\paragraph{Agent Behavior and Social Simulation}
\looseness=-1
LLM agents are increasingly used as human proxies in social simulation at scales from tens to thousands of individuals
\citep{park2023generative,park2024generative}, although persona-based simulations potentially risk flattening demographic representations and lack cognitively grounded reasoning beyond surface-level behavioral plausibility \citep{li2025llm,li2025simulating,wang2025large}.
Alignment research shows that explicit moral reward functions can teach agents cooperative strategies generalizing across game-theoretic environments \citep{tennant2025moral}.
Recent work measures the degree to which a model reasons about social concepts with the depth and critical rigor of a human expert \citep{watson2026scrub}.
However, current LLM fairness evaluation \citep{zhao2018gender,nangia2020crows,parrish2021bbq,smith2022m,tamkin2023evaluating,gallegos2024bias,gupta2024calm,rottger2025safetyprompts,fan2025fairmt} largely relies on standardized-test formats whose conclusions, as we demonstrate, could be dominated by prompt construction artifacts.
Our in-situ behavioral evaluation instead aims to identify stable, model-specific behavioral signatures that can generalize across benchmarks differing in fairness targets and methodologies.
